ACER: An AST-based Call Graph Generator Framework

We introduce ACER, an AST-based call graph generator framework. ACER leverages tree-sitter to interface with any language. We opted to focus on generators that operate on abstract syntax trees (ASTs) due to their speed and simplicitly in certain scenarios; however, a fully quantified intermediate representation usually provides far better information at the cost of requiring compilation. To evaluate our framework, we created two context-insensitive Java generators and compared them to existing open-source Java generators.

==> macros.tex <==
\makeatletter

% Approach name
\newcommand{\toolname}{{\sc MLCG}\xspace}
\newcommand{\toolnames}{{\sc MLCG's}\xspace}

% Dataset sizes:
\newcommand{\csnpairs}{\textcolor{red}{$XX$}\xspace}
\newcommand{\csnrepos}{\textcolor{red}{$XX$}\xspace}
\newcommand{\csncommits}{\textcolor{red}{$XX$}\xspace}
\newcommand{\csnreposfinal}{\textcolor{red}{$XX$}\xspace}

\newcommand{\imrepos}{\textcolor{black}{$25$}\xspace}
\newcommand{\imcommits}{\textcolor{black}{$910$}\xspace}
\newcommand{\imtasks}{\textcolor{red}{$XX$}\xspace}
% \newcommand{\originaldata}{$1,160,889$\xspace}

\newcommand{\tnew}[1]{{\bf { #1 }} }

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}

\definecolor{mycolor}{RGB}{204,204,204}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\small{\textbf{
			\node[shape=circle,fill=mycolor,draw=black, inner sep=0.75pt] (char) {\textcolor{black}{#1}};}}}}

\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }

\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etals}{\textit{et al.'s}\xspace}
\newcommand{\aka}{\textit{a.k.a.}\xspace}	
% \newcommand{\secref}[1]{Sec.~\ref{#1}\xspace}
% \newcommand{\chapref}[1]{Chapter~\ref{#1}\xspace}
\newcommand{\appref}[1]{Appendix~\ref{#1}\xspace}
% \newcommand{\figref}[1]{Fig.~\ref{#1}\xspace}
\newcommand{\listref}[1]{Listing~\ref{#1}\xspace}
\newcommand{\equaref}[1]{Equation~\ref{#1}\xspace}
\newcommand{\tabref}[1]{Table~\ref{#1}\xspace}

\newcommand\andrew[1]{{\color{red} \nb{ANDREW}{#1}}}
\newcommand\yanfu[1]{{\color{violet}\nb{YANFU}{#1}}}
\newcommand\denys[1]{{\color{blue}\nb{DENYS}{#1}}}

%\newcommand\NEW[1]{\nb{NEW}{#1}}
\newcommand\REF{{\color{red} REF}}
\newcommand\NEW[1]{{\color{black} #1}}
\newcommand\NEWR[1]{{\color{black} #1}}
\newcommand\NEWEST[1]{{\color{black} #1}}

\def\signed#1{{\unskip\nobreak\hfil\penalty50
    \hskip2em\hbox{}\nobreak\hfil\sl#1
    \parfillskip=0pt \finalhyphendemerits=0 \par}}
